Restereo: Diffusion stereo video generation and restoration

Stereo video generation has been gaining increasing attention with recent advancements in video diffusion models. However, most existing methods focus on generating 3D stereoscopic videos from monocular 2D videos. These approaches typically assume that the input monocular video is of high quality, making the task primarily about inpainting occluded regions in the warped video while preserving disoccluded areas. In this paper, we introduce a new pipeline that not only generates stereo videos but also enhances both left-view and right-view videos consistently with a single model. Our approach achieves this by fine-tuning the model on degraded data for restoration, as well as conditioning the model on warped masks for consistent stereo generation. As a result, our method can be fine-tuned on a relatively small synthetic stereo video datasets and applied to low-quality real-world videos, performing both stereo video generation and restoration. Experiments demonstrate that our method outperforms existing approaches both qualitatively and quantitatively in stereo video generation from low-resolution inputs.

==> commands.tex <==

% The next eight lines come directly from the completed rights form.
% You MUST replace them with the lines specific to your accepted work.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Use the "authoryear" citation style, and make sure citations are in [square brackets].
\citestyle{acmauthoryear}
\setcitestyle{nosort,square}

% A useful command for controlling the number of authors per row.
% The default value of "authorsperrow" is 2.
\settopmatter{authorsperrow=4}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% remove the following libaries for TAPS
\usepackage{mathrsfs}
\usepackage{tikz}
\usetikzlibrary{arrows.meta}
\usepackage{overpic}
\usepackage{pict2e}
\usepackage{dsfont}
\usepackage[most]{tcolorbox}
\usepackage[outline]{contour}
\usepackage{standalone}
\usepackage[normalem]{ulem}

\usepackage{microtype}      % betters typesetting
% \usepackage[capitalize]{cleveref}
\usepackage{xspace}         % proper spacing after macros
\usepackage{mathtools}      % \mathclap
\usepackage{nicefrac,xfrac} % nice fractions
% \usepackage{bm}             % proper bold math via \boldsymbol (\pmb is ugly!)
% \usepackage{bbm, dsfont}
% \usepackage{overpic}        % to draw stuff over images
% \usepackage{pict2e}         % to enable some fractional coordinates when drawing with overpic
\usepackage{mathtools}

% \usepackage{MnSymbol}  % for arrow symbols used in algorithm comments
\usepackage{stmaryrd}  % for \sswarrow and \nnearrow in algorithm comments
\usepackage{newfloat}  % for declaring custom environments
\usepackage{savesym}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode} 
\algrenewcommand\textproc{}
\usepackage{graphicx}
% \usepackage{tikz}
\usepackage{grffile}  % to be able to use images with periods in their file names, without specifying the file extensions
\usepackage{soul}
\usepackage{wrapfig}
\usepackage{bbm}
\usepackage{flushend}
% \usepackage[capitalize]{cleveref}
\usepackage{tabularx}
\usepackage{ctable}            % nicer tables
% \usepackage{mathrsfs}
% \usepackage[most]{tcolorbox}   % for boxes around equations
\usepackage[a]{esvect}           % nice over-arrow (for vectors) using \vv{a}
% \usepackage{MnSymbol}          % for arrow symbols used in algorithm comments
% \usepackage[outline]{contour}  % to make outlined text
% \usepackage{transparent}       % making text semi-transparent (gives compilation errors though...)
\usepackage{multirow}

\usepackage{wrapfig}
\usepackage{textcomp}    % for \textregistered
\usepackage{enumitem}    % to control the leftmargin in itemize


% \usepackage[ruled,vlined]{algorithm2e}

% \hypersetup{draft} % temporarily disable hyperlinks

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colors
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\definecolor{Red}{rgb}{1,0.45,0.45}
\definecolor{Green}{rgb}{0.44,0.76,0.33}
\definecolor{Blue}{rgb}{0.46,0.7,1}
\definecolor{DarkGreen}{rgb}{0.0,0.6,0.0}
\definecolor{DomainColor}{gray}{0}
\definecolor{ExtSpaceColor}{rgb}{0.86,0,0.86}
\definecolor{ExtSpaceColorTwo}{rgb}{0.86,0.5,0.86}
\definecolor{TargetSpaceColor}{hsb}{0.45,0.87,0.81}
\definecolor{TargetMeasureColor}{rgb}{0.3,0.3,0.3}
% \definecolor{TargetSpaceColor}{rgb}{0.8,0.5,0.07}
\definecolor{RedClassColor}{hsb}{0.99,0.62,0.9}
\definecolor{BlueClassColor}{hsb}{0.61,0.6,0.9}
\definecolor{PurpleClassColor}{rgb}{0.86,0.35,0.88}
\definecolor{ProjectionColor}{rgb}{0.95,0.57,0.00}
% NSColor(calibratedHue: 0.61, saturation: 0.60, brightness: 1.00, alpha: 1.000)
% NSColor(calibratedHue: 0.99, saturation: 0.62, brightness: 0.99, alpha: 1.000)
% NSColor(calibratedHue: 0.45, saturation: 0.87, brightness: 0.81, alpha: 1.000)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\unsure}[1]{{\sethlcolor{yellow}\hl{#1}}}

\newcommand{\Ignore}[1]{#1}  % use to include comments
%\newcommand{\Ignore}[1]{}  % use to exclude comments
%\mymath{\Ignore}[1]{}   % use to remove comments
\newcommand{\commentOutText}[1]{}
%% Comments
\newcommand{\todo}[1]{\Ignore{\textcolor[rgb]{0.9,0.2,0.6}{[#1]}}}
\newcommand{\gurprit}[1]{\Ignore{\textcolor[rgb]{1,0.27,0}{\textit{[Gurprit: #1]}}}}
\newcommand{\corentin}[1]{\Ignore{\textcolor[rgb]{0.13,0.54,0.13}{\textit{[Corentin: #1]}}}}
\newcommand{\xingchang}[1]{\Ignore{\textcolor[rgb]{0.627, 0.125, 0.941}{\textit{[Xingchang: #1]}}}}
\newcommand{\cengiz}[1]{\Ignore{\textcolor[rgb]{1,0,1}{\textit{[Cengiz: #1]}}}}
\newcommand{\cristina}[1]{\Ignore{\textcolor[rgb]{1,0.5,0.1}{\textit{[Cristina: #1]}}}}
% \newcommand{\revision}[1]{\Ignore{\textcolor[rgb]{0.1, 0.1, 1.0}{#1}}}
\newcommand{\revision}[1]{\Ignore{\textcolor[rgb]{0.0, 0.0, 0.0}{#1}}}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\Eg}{E.g.,\xspace}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\wrt}{w.r.t.\xspace}

%% Paper structure
\newcommand{\Paragraph}[1]{\paragraph{#1}}
% \mymath{\Paragraph}[1]{\subsubsection*{#1}}

%% Equation scaling
\newcommand{\ScaleMath}[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}

\newcommand{\mymath}[2]{\newcommand{#1}{\TextOrMath{$#2$\xspace}{#2}}}

% Equation emphasis - from the transmittance paper
% \tcbset{
%     % colback=yellow!5!white,
%     colback=white!98!black,
%     colframe=white!75!black,
%     boxrule=0.15mm,
%     arc=0.3mm,
%     boxsep=0pt,left=2pt,right=4pt,top=2pt,bottom=4pt
% }

%% Code listings
\savesymbol{Comment}
\algrenewcommand\algorithmicindent{3mm}
\captionsetup[algorithm]{labelsep=period}

%% Custom pseudocode environment (use in leu of algorithm environment)
\DeclareFloatingEnvironment[
    name=Alg.,
    placement=tbhp,
    within=none,
]{pseudocode}
\crefname{pseudocode}{Alg.}{Algs.}
\Crefname{pseudocode}{Algorithm}{Algorithms}

%% Commenrs in algorithm environment
\newcommand{\AlgCommentTemplate}[2]{\hfill{\fontsize{9} {6}\selectfont\textcolor{DarkGreen}{\text{#1\;#2}}}}
\newcommand{\AlgComment}[1]{\AlgCommentTemplate{}{#1}}
\newcommand{\AlgCommentLeft}[1]{\AlgCommentTemplate{$\pmb{\leftarrow}$}{#1}}
% \newcommand{\AlgCommentDown}[1]{\AlgCommentTemplate{$\pmb{\rcurvearrowsw}$}{#1}}
\newcommand{\AlgCommentDown}[1]{\AlgCommentTemplate{$\pmb{\sswarrow}$}{#1}}
% \newcommand{\AlgCommentUp}[1]{\AlgCommentTemplate{\reflectbox{\pmb{\rcurvearrowne}}}{#1}}
% \newcommand{\AlgCommentUp}[1]{\AlgCommentTemplate{\reflectbox{$\pmb{\rcurvearrowne}$}}{#1}}
\newcommand{\AlgCommentUp}[1]{\AlgCommentTemplate{\reflectbox{$\pmb{\nnearrow}$}}{#1}}

%% To be able to include Illustrator files as PDFs
\DeclareGraphicsRule{.ai}{pdf}{.ai}{}

%% When including images, prioritize vector graphics, then JPEG, then PNG
\DeclareGraphicsExtensions{.ai,.pdf,.jpg,.png}


%% Text with outline; params are [text color][outline color][thickness]{text}
\DeclareDocumentCommand{\Outlined}{ O{black} O{white} O{0.55pt} m }{%
    \contourlength{#3}% how thick each copy is
    % \contournumber{30}% number of copies, when not using the [outline]{contour} option
    % \transparent{#4}{\contour{#2}{\small \textcolor{#1}{\textsf{#5}}}}%
    \contour{#2}{\textcolor{#1}{#4}}%
}

% To undefine a color; useful when reusing colors, e.g. TextColor, OutlineColor, etc.
\newcommand{\undefinecolor}[1]{\expandafter\let\csname\string\color@#1\endcsname\undefined}


% {iamge}{width}{caption}{verticalspace}
\newcommand{\mywfigurevspace}[4]{%

\begin{wrapfigure}{r}{#2\columnwidth}%
 \hspace{-0.7cm}%
 \vspace{#4}%
    \centering
    \includegraphics[width=#2\columnwidth]{#1}%
    \vspace{-.2cm}%
    % \caption{#3}%
    \label{fig:#1}%
    \vspace{-0.3cm}% 
\end{wrapfigure}%
%\leavevmode%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% math
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mymath{\NumFrames}{F}












==> figures/ablation_data_augmentation_onerow.tex <==
%!TEX root = ../main.tex

% \newcommand{\PlotSingleImage}[1]{%
%     % \begin{tikzpicture}[scale=1.165]
%         \begin{scope}
%             \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
%             \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
%         \end{scope}
%         \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
%     % \end{tikzpicture}%
% }


\newcommand{\PlotSingleImage}[1]{%
    \begin{tikzpicture}[scale=1.15]    % 1.165
        \begin{scope}
            \clip (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
        
    \end{tikzpicture}%
}


\newcommand\scalevalue{1.2}    % 0.65
%
\small
% \hspace*{-2mm}
% \begin{tabular}{c@{\;}}
\begin{tabular}{c@{\;}c@{\;}c@{}}
% Input video from SVD~\cite{blattmann2023stable} (15th frame)
Input video from Pixabay~\cite{pixabay2025}
& 
Ours left (wo/ augmentation)
& 
Ours left (w/ augmentation)
\\

% \rotatebox{90}{\hspace{0.1cm} \small Input}
% &
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{results_ours/pixabay_dice2/pixabay_dice2_input_left_00015.png}
% \PlotSingleImage{results_ours/pixabay_teapot/pixabay_teapot_input_left_00012.png}
\end{tikzpicture}

% \\

% \rotatebox{90}{\hspace{0.5cm} \small Ours left (wo/ aug)}
&
\begin{tikzpicture}[scale=\scalevalue]
%\PlotSingleImage{results_ours_noaug/svd_robot/svd_robot_ours_0.03_left_00015.png}
\PlotSingleImage{results_ours_noaug/pixabay_dice2/pixabay_dice2_ours_0.03_left_00015.png}
% \PlotSingleImage{results_ours_noaug/pixabay_turtle1/pixabay_turtle1_ours_0.03_left_00014.png}
\end{tikzpicture}

% \\

% \rotatebox{90}{\hspace{0.0cm} \small Ours left (w/ aug)}
&
\begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImage{results_ours/svd_robot/svd_robot_ours_0.03_left_00015.png}
\PlotSingleImage{results_ours/pixabay_dice2/pixabay_dice2_ours_0.03_left_00015.png}

\end{tikzpicture}

\\
[-0.4mm]
% \end{tabular}
\end{tabular}



==> figures/depth_gt_vs_depth_crafter.tex <==
%!TEX root = ../main.tex

% \newcommand{\PlotSingleImage}[1]{%
%     % \begin{tikzpicture}[scale=1.165]
%         \begin{scope}
%             \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
%             \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
%         \end{scope}
%         \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
%     % \end{tikzpicture}%
% }


\newcommand{\PlotSingleImage}[1]{%
    \begin{tikzpicture}[scale=1.1]    % 1.165, 1.15
        \begin{scope}
            \clip (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
        
    \end{tikzpicture}%
}


\newcommand\scalevalue{1.2}    % 0.65
%
\small
\hspace*{-4mm}
% \begin{tabular}{c@{\;}}
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{}}
% \rotatebox{90}{\hspace{0.8cm} \small MVDream}
& Input & Trained with DepthCrafter & Trained with ground truth depth 
\\
% [-0.4mm]
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{depth_gt_vs_depth_crafter/00000.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{depth_gt_vs_depth_crafter/depth_crafter/sora_monster_ours_0.03_right_00000.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{depth_gt_vs_depth_crafter/depth_gt/sora_monster_ours_0.03_right_00000.png}
\end{tikzpicture}
\\
[-0.4mm]
% \end{tabular}
\end{tabular}


==> figures/histogram_matching.tex <==
%!TEX root = ../main.tex

% \newcommand{\PlotSingleImage}[1]{%
%     % \begin{tikzpicture}[scale=1.165]
%         \begin{scope}
%             \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
%             \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
%         \end{scope}
%         \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
%     % \end{tikzpicture}%
% }


\newcommand{\PlotSingleImage}[1]{%
    \begin{tikzpicture}[scale=1.2]    % 1.165
        \begin{scope}
            \clip (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
        
    \end{tikzpicture}%
}


\newcommand\scalevalue{1.2}    % 0.65
%
\small
\hspace*{4mm}
% \begin{tabular}{c@{\;}}
\begin{tabular}{c@{\;}c@{}}
% \rotatebox{90}{\hspace{0.8cm} \small MVDream}
& Video from pixabay[] (1st frame)

\\

\rotatebox{90}{\hspace{0.1cm} \small Input}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{results_ours/pixabay_flower/pixabay_flower_input_left_00000.png}
\end{tikzpicture}

\\

\rotatebox{90}{\hspace{0.5cm} \small Ours left}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{results_ours/pixabay_flower/pixabay_flower_ours_0.03_left_00000.png}
\end{tikzpicture}

\\

\rotatebox{90}{\hspace{0.0cm} \small Ours right (wo/ hist)}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{results_ours/pixabay_flower/pixabay_flower_ours_0.03_right_00000.png}
\end{tikzpicture}

\\

\rotatebox{90}{\hspace{0.0cm} \small Ours right (w/ hist)}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{results_ours/pixabay_flower/pixabay_flower_ours_0.03_right_hist_00000.png}
\end{tikzpicture}

\\
[-0.4mm]
% \end{tabular}
\end{tabular}



==> figures/old_ablation_data_augmentation.tex <==
%!TEX root = ../main.tex

% \newcommand{\PlotSingleImage}[1]{%
%     % \begin{tikzpicture}[scale=1.165]
%         \begin{scope}
%             \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
%             \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5cm,2.5cm);
%         \end{scope}
%         \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
%     % \end{tikzpicture}%
% }


\newcommand{\PlotSingleImage}[1]{%
    \begin{tikzpicture}[scale=1.3]    % 1.165
        \begin{scope}
            \clip (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/#1] (0,0) rectangle (5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
        
    \end{tikzpicture}%
}


\newcommand\scalevalue{1.2}    % 0.65
%
\small
\hspace*{4mm}
% \begin{tabular}{c@{\;}}
\begin{tabular}{c@{\;}c@{}}
% \rotatebox{90}{\hspace{0.8cm} \small MVDream}
& Video from SVD~\cite{blattmann2023stable} (15th frame)

\\

\rotatebox{90}{\hspace{0.1cm} \small Input}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{results_ours/svd_robot/svd_robot_input_left_00015.png}
\end{tikzpicture}

\\

\rotatebox{90}{\hspace{0.5cm} \small Ours left (wo/ aug)}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{results_ours_noaug/svd_robot/svd_robot_ours_0.03_left_00015.png}
\end{tikzpicture}

\\

\rotatebox{90}{\hspace{0.0cm} \small Ours left (w/ aug)}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImage{results_ours/svd_robot/svd_robot_ours_0.03_left_00015.png}
\end{tikzpicture}

\\
[-0.4mm]
% \end{tabular}
\end{tabular}



==> figures/old_comparison_stereo_crop_v0.tex <==
%!TEX root = ../main.tex

% \newcommand{\PlotSingleImageBB}[1]{%
%     \begin{tikzpicture}[scale=1.1] % Adjust overall scale if needed
%         % Full image viewport (using the same clipping as before)
%         \begin{scope}
%             \clip (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
%             \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%         \end{scope}
%         % Draw the full image border
%         \draw (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
%         % Overlay a red bounding box for the crop region
%         \draw[line width=1pt, red] (1.25,0) rectangle (3.75,2.5);
%     \end{tikzpicture}%
% }


% \newcommand{\PlotCroppedImageEnlarged}[1]{
%     \begin{tikzpicture}[scale=1.1]
%         \begin{scope}
%             \clip (1.25,0) rectangle (3.75,2.5);
%             \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%         \end{scope}
%         \draw (1.25,0) rectangle (3.75,2.5);
%         % \begin{scope}
%         %     \clip (3.75,0) rectangle (5.25,2.5);
%         %     \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%         % \end{scope}
%         % \draw (3.75,0) rectangle (5.25,2.5);
%     \end{tikzpicture}
%     \begin{tikzpicture}[scale=1.1]
%         \begin{scope}
%             \clip (3.75,0) rectangle (5.25,2.5);
%             \path[fill overzoom image=figures/#1] (2.5,0) rectangle (7.5,2.5);
%         \end{scope}
%         \draw (3.75,0) rectangle (5.25,2.5);
%     \end{tikzpicture}
% }


% \newcommand{\PlotCroppedImageEnlarged}[1]{%
%   \hspace{4.6em}%
%     % First crop: corresponding to the first bounding box.
%     \begin{tikzpicture}[scale=1.1, baseline]
%       \begin{scope}
%         \clip (0.4,0.6) rectangle (2.8,1.8);
%         \begin{scope}[transform canvas={scale=1}]%
%           \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%         \end{scope}
%       \end{scope}
%       \draw (0.4,0.6) rectangle (2.8,1.8);
%     \end{tikzpicture}%
%     \hspace{0.5em}%
%     % Second crop: using the same vertical span.
%     \begin{tikzpicture}[scale=1.1, baseline]
%       \begin{scope}
%         \clip (2.6,0.3) rectangle (5.0,1.5);
%         \begin{scope}[transform canvas={scale=1}]%
%           \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%         \end{scope}
%       \end{scope}
%       \draw (2.6,0.3) rectangle (5.0,1.5);
%     \end{tikzpicture}%
% }


\newcommand{\PlotSingleImageBB}[1]{%
    \begin{tikzpicture}[scale=1.1]
        \begin{scope}
            \clip (0,0) rectangle (5,2.5);
            \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
        \end{scope}
        \draw (0,0) rectangle (5,2.5);
        % first box
        \draw[line width=1pt, red] (0.4,0.6) rectangle (2.8,1.8);
        % second box
        \draw[line width=1pt, red] (2.6,0.3) rectangle (5.0,1.5);
    \end{tikzpicture}%
}


\newcommand{\PlotCroppedImageEnlarged}[1]{%
\hspace{1.4em}
  \begin{tikzpicture}[scale=1.1, baseline=(baselineNode.south)]
    % A reference node for baseline alignment
    \coordinate (baselineNode) at (0,0);

    %---------------------------------------
    % First crop (bounding box: (0.4,0.6)–(2.8,1.8))
    %---------------------------------------
    \begin{scope}[xshift=0cm, yshift=0cm] % place it at (0,0)
      \clip (0.4,0.6) rectangle (2.8,1.8);
      
    \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
      
      \draw (0.4,0.6) rectangle (2.8,1.8);
    \end{scope}

    %---------------------------------------
    % Second crop (bounding box: (2.6,0.3)–(5.0,1.5))
    %---------------------------------------
    % If you want it to appear horizontally aligned with the first,
    % shift it so the bottom edges line up visually.
    \begin{scope}[xshift=0.3cm, yshift=0.3cm]
      \clip (2.6,0.3) rectangle (5.0,1.5);
      \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
      \draw (2.6,0.3) rectangle (5.0,1.5);
    \end{scope}

  \end{tikzpicture}%
}


 



\newcommand\scalevalue{1.2} % Adjust overall size in the table if needed

\small
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{}}
& Video from~\citet{li2024generative} (3rd frame) & Video from CLEVER~\cite{johnson2017clevr} (11th frame) & Video from [] (6th frame)
\\
% [2mm]
\rotatebox{90}{\hspace{0.1cm}\small Input left videos}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageBB{results_ours/gid_grapes/gid_grapes_input_left_00002}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageBB{results_ours/clever_video_10010/clever_video_10010_input_left_00009.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageBB{results_ours/pixabay_book/pixabay_book_input_left_00005} 
\end{tikzpicture}
\\
% [2mm] % space between rows
\rotatebox{90}{\hspace{0.1cm}\small cropped}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotCroppedImageEnlarged{results_ours/gid_grapes/gid_grapes_input_left_00002}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotCroppedImageEnlarged{results_ours/clever_video_10010/clever_video_10010_input_left_00009.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotCroppedImageEnlarged{results_ours/pixabay_book/pixabay_book_input_left_00005}
\end{tikzpicture}
\\[-0.4mm]
\end{tabular}


==> figures/old_comparison_stereo_crop_vertical.tex <==
%!TEX root = ../main.tex

% \newcommand{\PlotSingleImageBB}[1]{%
%     \begin{tikzpicture}[scale=1.1] % Adjust overall scale if needed
%         % Full image viewport (using the same clipping as before)
%         \begin{scope}
%             \clip (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
%             \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%         \end{scope}
%         % Draw the full image border
%         \draw (0,0) -- (5,0) -- (5,2.5) -- (0,2.5) -- cycle;
%         % Overlay a red bounding box for the crop region
%         \draw[line width=1pt, red] (1.25,0) rectangle (3.75,2.5);
%     \end{tikzpicture}%
% }


% \newcommand{\PlotCroppedImageEnlarged}[1]{
%     \begin{tikzpicture}[scale=1.1]
%         \begin{scope}
%             \clip (1.25,0) rectangle (3.75,2.5);
%             \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%         \end{scope}
%         \draw (1.25,0) rectangle (3.75,2.5);
%         % \begin{scope}
%         %     \clip (3.75,0) rectangle (5.25,2.5);
%         %     \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%         % \end{scope}
%         % \draw (3.75,0) rectangle (5.25,2.5);
%     \end{tikzpicture}
%     \begin{tikzpicture}[scale=1.1]
%         \begin{scope}
%             \clip (3.75,0) rectangle (5.25,2.5);
%             \path[fill overzoom image=figures/#1] (2.5,0) rectangle (7.5,2.5);
%         \end{scope}
%         \draw (3.75,0) rectangle (5.25,2.5);
%     \end{tikzpicture}
% }


% \newcommand{\PlotCroppedImageEnlarged}[1]{%
%   \hspace{4.6em}%
%     % First crop: corresponding to the first bounding box.
%     \begin{tikzpicture}[scale=1.1, baseline]
%       \begin{scope}
%         \clip (0.4,0.6) rectangle (2.8,1.8);
%         \begin{scope}[transform canvas={scale=1}]%
%           \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%         \end{scope}
%       \end{scope}
%       \draw (0.4,0.6) rectangle (2.8,1.8);
%     \end{tikzpicture}%
%     \hspace{0.5em}%
%     % Second crop: using the same vertical span.
%     \begin{tikzpicture}[scale=1.1, baseline]
%       \begin{scope}
%         \clip (2.6,0.3) rectangle (5.0,1.5);
%         \begin{scope}[transform canvas={scale=1}]%
%           \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%         \end{scope}
%       \end{scope}
%       \draw (2.6,0.3) rectangle (5.0,1.5);
%     \end{tikzpicture}%
% }


\newcommand{\PlotSingleImageBB}[1]{%
    \begin{tikzpicture}[scale=1.1]
        \begin{scope}
            \clip (0,0) rectangle (5,2.5);
            \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
        \end{scope}
        \draw (0,0) rectangle (5,2.5);
    \end{tikzpicture}%
}



% Command to display two cropped images
\newcommand{\PlotCroppedImageEnlarged}[2]{%
  \centering
  \begin{tikzpicture}[scale=1.1]
    % First crop: occupies the left half, size: 2.5 (width) x 1.25 (height)
    \begin{scope}
      \clip (0,0) rectangle (2.5,1.25);
      \path[fill overzoom image=figures/#1] (0,0) rectangle (2.5,1.25);
    \end{scope}
    \draw[thick] (0,0) rectangle (2.5,1.25);
    
    % Second crop: shifted right by 2.5, occupies the right half, size: 2.5 x 1.25
    \begin{scope}[xshift=2.5cm]
      \clip (0,0) rectangle (2.5,1.25);
      \path[fill overzoom image=figures/#2] (0,0) rectangle (2.5,1.25);
    \end{scope}
    \draw[thick] (2.5,0) rectangle (5,1.25);
  \end{tikzpicture}%
}
% \newcommand{\PlotCroppedImageEnlarged}[1]{%
% \hspace{1.4em}
%   \begin{tikzpicture}[scale=1.1, baseline=(baselineNode.south)]
%     % A reference node for baseline alignment
%     \coordinate (baselineNode) at (0,0);

%     %---------------------------------------
%     % First crop (bounding box: (0.4,0.6)–(2.8,1.8))
%     %---------------------------------------
%     \begin{scope}[xshift=0cm, yshift=0cm] % place it at (0,0)
%       \clip (0.4,0.6) rectangle (2.8,1.8);
      
%     \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
      
%       \draw (0.4,0.6) rectangle (2.8,1.8);
%     \end{scope}

%     %---------------------------------------
%     % Second crop (bounding box: (2.6,0.3)–(5.0,1.5))
%     %---------------------------------------
%     % If you want it to appear horizontally aligned with the first,
%     % shift it so the bottom edges line up visually.
%     \begin{scope}[xshift=0.3cm, yshift=0.3cm]
%       \clip (2.6,0.3) rectangle (5.0,1.5);
%       \path[fill overzoom image=figures/#1] (0,0) rectangle (5,2.5);
%       \draw (2.6,0.3) rectangle (5.0,1.5);
%     \end{scope}

%   \end{tikzpicture}%
% }


 



\newcommand\scalevalue{1.2} % Adjust overall size in the table if needed

\small
\begin{tabular}{c@{\;}c@{\;}c@{\;}c@{}}
& Video from~\citet{li2024generative} (3rd frame) & Video from CLEVER~\cite{johnson2017clevr} (11th frame) & Video from [] (6th frame)
\\
% [2mm]
\rotatebox{90}{\hspace{0.1cm}\small Input left videos}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageBB{results_ours_crop/gid_grapes/gid_grapes_input_left_00002_with_boxes.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotSingleImageBB{results_ours_crop/gid_grapes/gid_grapes_input_left_00002_with_boxes.png}
\end{tikzpicture}
&
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotSingleImageBB{results_ours/pixabay_book/pixabay_book_input_left_00005} 
% \end{tikzpicture}
\\

\rotatebox{90}{\hspace{0.1cm}\small cropped}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotCroppedImageEnlarged{results_ours_crop/gid_grapes/gid_grapes_input_left_00002_crop1.png}{results_ours_crop/gid_grapes/gid_grapes_input_left_00002_crop2.png}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalue]
\PlotCroppedImageEnlarged{results_ours_crop/gid_grapes/gid_grapes_input_left_00002_crop1.png}{results_ours_crop/gid_grapes/gid_grapes_input_left_00002_crop2.png}
\end{tikzpicture}
&
% \begin{tikzpicture}[scale=\scalevalue]
% \PlotCroppedImageEnlarged{results_ours/pixabay_book/pixabay_book_input_left_00005}
% \end{tikzpicture}
\\[-0.4mm]
\end{tabular}

